Constrained Reinforcement Learning and Formal Verification for Safe Colonoscopy Navigation

The field of robotic Flexible Endoscopes (FEs) has progressed significantly, offering a promising solution to reduce patient discomfort. However, the limited autonomy of most robotic FEs results in non-intuitive and challenging manoeuvres, constraining their application in clinical settings. While previous studies have employed lumen tracking for autonomous navigation, they fail to adapt to the presence of obstructions and sharp turns when the endoscope faces the colon wall. In this work, we propose a Deep Reinforcement Learning (DRL)-based navigation strategy that eliminates the need for lumen tracking. However, the use of DRL methods poses safety risks as they do not account for potential hazards associated with the actions taken. To ensure safety, we exploit a Constrained Reinforcement Learning (CRL) method to restrict the policy in a predefined safety regime. Moreover, we present a model selection strategy that utilises Formal Verification (FV) to choose a policy that is entirely safe before deployment. We validate our approach in a virtual colonoscopy environment and report that out of the 300 trained policies, we could identify three policies that are entirely safe. Our work demonstrates that CRL, combined with model selection through FV, can improve the robustness and safety of robotic behaviour in surgical applications.

==> Unused_text.tex <==
Abstract:
The development of robotic Flexible Endoscope (FEs) technologies have made significant progress and present a viable alternative towards reduced patient discomfort. However, low autonomy level of most robotic FEs leads to nonintuitive and difficult manipulations, which limits their applications in clinical practice.
Prior works on autonomous navigation used lumen tracking to guide the navigation; however they fail to adapt under the presence of occlusion and at sharp turns when the endoscope faces the colon wall. 
This work presents an autonomous navigation strategy based on Deep Reinforcement Learning (DRL) that is independent of lumen tracking.  DRL methods are known to pose safety challenge since they do do not consider the risks associated with the actions.
To tackle the issue of safety, we propose a safe-RL framework that use constrained policy optimisation to restrict the policy in a predefined safety regime. Furthermore, we provide a model selection strategy that uses formal verification to select policy which is absolutely safe prior to deployment of the agent. 
We validate our approach in a virtual colonoscopy environment. Our results showed that we could find 3 policies out of 300 policies trained that are completely safe.
Constrained policy optimisation in addition to model selection through FV can pave a way towards increased robust and safe robotic behaviour in the surgical domain.

Introduction:

1.9 million new cases of ColoRectal Cancer (CRC) were detected worldwide in 2020 with a mortality of 935 thousand people \cite{sung2021global}. The World Health Organization (WHO) estimates an average increase rate of 3\% per year globally for the next 20 years \cite{observatory}. 
Early stage detection is key to increase the survival rate, which is close to 100\% at Stage 0 and goes down below 5\% at Stage IV \cite{van2014conditional}.
Colonoscopy screening programs are widely adopted examination procedures for diagnosing and treating CRC, where a flexible endoscope equipped with an optical camera and light source, is manually inserted to perform inspection \cite{ciuti2020frontiers, manfredi2021endorobots}. There are two major drawbacks of this routine
(i) patients without sedation need to undertake great discomfort and pain due to the forcible insertion that leads to tissue stretching. 
A common issue is scope looping, where the colonoscope continues to advance into the colon without a simultaneous progression of the tip, thus distending the colon and causing 90\% of the patient pain experienced during procedures \cite{formosa2019novel}, increasing the risk of colon perforation and massive bleeding \cite{kim2019adverse} (ii) nonintuitive and difficult manipulation of the flexible endoscopes requires extremely high skills for the clinicians. A shortage of endoscopists with respect to demand leads to increased physical stress and muscoskeletal injuries \cite{martin2020enabling}.

% In addition, the employment of a soft tether in some robotic colonoscopes can achieve a more gentle interaction between the colonoscope and colon wall, which is helpful to eliminate the problem of tissue stretching.

% The development of robotic endoscopes introduced a painless alternative to inspect the GastroIntestinal (GI) tract. Different active locomotion such as magnetically guided wireless capsule and endoscope \cite{xu2022autonomous, huang2021autonomous}, treaded capsule and endoscope \cite{formosa2019novel} and legged propulsion \cite{lee2019reel} to actuate the colonoscope.
% The fact that manual navigation systems are highly susceptible to human error and require that operators undergo extensive training has prompted
% development in autonomous navigation systems for endoscopy \cite{martin2020enabling}.


A wide range of attempts have been made to develop autonomous visual navigation solutions for flexible and capsule endoscopes to advance through the lumen. 
These approaches assume that the region of greatest depth within any given image represents a useful goal for immediate heading adjustment \cite{van2014image}.
Lumen depth estimation using the edges or contours of structures surrounding the lumen has been demonstrated \cite{prendergast2018autonomous, mathew2021foldit, prendergast2020real}. However, large structures like haustral folds may not always be present in images, particularly under the presence of occlusion
and during sharp turns when an endoscope faces the colon wall for much of the maneuver.
The most common methods for finding the greatest depth have focused on darkest or deepest region techniques in which the darkest and/or deepest region in an image is identified and used as the goal for adjusting endoscope heading.
These techniques are typically simple to execute and many studies have examined different techniques for both segmentation of these dark regions and 3-D depth estimation utilising shape-from-shading or structured light approaches \cite{reilink2010image,van2014image, martin2020enabling}. 
All the above mentioned methods require user-defined visual features which are generally cumbersome to hand-engineer. Lazo \textit{et al.} developed a convolution neural network (CNN) based approach for lumen segmentation that does not require hand-crafted solution and tend to generalise better when they are trained in a large enough amount of data \cite{lazo2022autonomous}.

However, a major concern with implementing DRL in real-world, unstructured environments is safety, which is of utmost priority in surgical settings. DRL methods are prone to exhibiting unanticipated behavior in states not encountered during training, which can lead to catastrophic consequences \cite{GoShSz15, GaFe15}.

Once the lumen centre is computed, a rule based controller such as the proportional, integral, derivative (PID) controller is used to reduce the distance between the image centre and the detected lumen centre \cite{lazo2022autonomous, martin2020enabling, prendergast2018autonomous}. Rule-based controllers do not possess the ability to adapt and therefore sudden changes in the environment can lead to their failure. 
DRL has been one of the proposed methods to generate adaptive control, which can provide an end-to-end mapping between the endoscopic images and the control signal of the endoscope \cite{pore2022colonoscopy}. The reward function used motivates the agent to reduce the lumen distance, which itself requires a perception system for lumen detection. 
Therefore, in this work we focus on developing a DRL methodology that is independent from a separate perception system.
However, one of major concerns with implementing DRL in real world robot in an unstructured environment system is safety, which is one of the utmost priorities during a surgery. DRL methods are prone to show unanticipated behaviour in states not encountered during training which in cases can lead to catastrophic consequences \cite{GoShSz15, GaFe15}.

%Constrained Reinforcement Learning (CRL) provides a way to tackle safety by embedding the environment with cost functions that restrict the agents from taking certain actions. Several techniques have been developed to optimize the reward function while maintaining the cost below a specified threshold. 

In literature, a wide variety of algorithms have been developed to find policies that, at the same time, maximize the reward function, while keeping the cost below a given threshold. Some examples are IPO \cite{LiDiLi20}, which exploits a logarithmic barrier function for the optimization, CPO \cite{AcHeTa17}, which is based on the concept of safe policy improvement inherited from TRPO \cite{ShLeAb15}, and other techniques, such as SOS \cite{MaCoFa21b}, that propose to perform a genetic step to increase the safety inside the training loop.
Among all these approaches, in this paper, we focus on Lagrangian-PPO (LPPO) \cite{StAcAb20}, which exploits the lagrangian dual relaxation of a constrained optimization problem, to obtain a simple and effective algorithm, that shows excellent results in a wide variety of tasks \cite{RaAcAm19}.

The safety specifications in common constrained RL methods are expected discounted cumulative costs, which average the potential danger at a state to the whole trajectory. Therefore, constraints imposed on expected cumulative costs lack rigorous definitions and guarantee of safety \cite{yu2022reachability}.
Hence ensuring that the agent never makes decisions that can cause safety violation is crucial. Such validation requires estimating the violation without actually executing the action. Running the network over many experiments and collecting the unsafe configurations can be time-consuming and can only give an empirical evaluation without any guarantee of safety \cite{Liu}. Therefore, in this paper, we exploit the concept of Formal Verification (FV) to provide mathematical guarantees that ensure that the agent actions lie in the safe regime, before the deployment of the trained agent. 
However, due to the high-dimensional, non-linear, and the complex structure of Deep Neural Networks (DNN) used in DRL, providing formal guarantees on them is a challenging NP-Hard problem \cite{Reluplex}.
%is a challenging task, that has proven to be NP-Hard \cite{Reluplex}. 

% In the last years, a lot of work has been done to develop novel tools that can handle different types of formal verification, such as FV for real-world neural networks \cite{Marabou, Eh17, WaZhXu21}, quantitative verification \cite{baluta2019quantitative, CountingProVe}, and in particular, FV for DRL agents that involve multiple interactions with the environment in an iterative decision-making process \cite{ProVe, TACAS}.
% Therefore, in this work, we exploit VeriNet, a state-of-the-art sound and complete formal verification tool \cite{Verinet1, Verinet2}, to develop a model selection framework that allows us to guarantee that the final model is completely safe against the required properties. 
% Crucially, from our experiments, we found that such a model does not exist among the agent trained with the standard version of PPO. In contrast, from the constrained DRL process, we obtain four provably safe agents.

Several studies have developed novel tools that can handle different types of FV for real-world neural networks \cite{Marabou, Eh17, WaZhXu21} and quantitative verification \cite{baluta2019quantitative, CountingProVe}. Recently, FV has been adapted to the DRL setup, that involve multiple interactions with the environment in an iterative decision-making process \cite{ProVe, TACAS}. These tools were applied for robot-assisted surgical tasks to identify states that can cause safety violations \cite{pore2021learning}, however the guarantee of the overall safety behaviour of the robot was not provided. In this work, we exploit VeriNet, a state-of-the-art sound and complete formal verification tool \cite{Verinet1, Verinet2}, to develop a model selection strategy that allows us to guarantee that the final model is completely safe against the required properties. 


% Our main contributions are:
% (1) we develop a DRL method which does not require the need for a lumen detection system
% (2) we provide a safe-RL framework based on constrained policy optimisation to constrain the policy in a safe state-space that follows pre-defined safety criteria.
% (3) A model selection strategy that can select policies which satisfy all the safety constraints. Each policy is formally verified to check its safety violations.

The 3D models of the colon are extracted from a public CT colonography dataset and refined to apply volumetric and superficial meshes with realistic textures applied using the real endoscopy images from the KVASIR dataset \cite{incetan2021vr,pore2022colonoscopy}. The obtained colon models are loaded in \textit{SOFA (Simulation Open Framework Architecture)} to generate a mechanical model to mimic the deformable nature of the colon.
\textit{Unity3D} is adopted to create high quality realistic rendering and to create mesh colliders to detect collisions with the endoscope \cite{tagliabue2020soft}.

% The collision with the wall is detected using the mesh collision system provided by Unity3D. A collision is detected when an intersection between the bounds of the two meshes is detected.

% The 3D models of the bowel are segmented in a semi-automated way using a public CT colonography dataset \cite{incetan2021vr}. The segmented models are refined, and volumetrical and superficial meshes are generated. Realistic textures are created and applied to the models using the real endoscopy images from KVASIR dataset \cite{incetan2021vr}. Then, the obtained colon models are loaded into \textit{SOFA (Simulation Open Framework Architecture)}, where a realistic mechanical model based on real-time finite element analysis is generated, setting the simulation parameters in order to mimic the colon tissue behaviour \cite{christensen2015tensile}. Additionally, the collision detection between the endoscope and the colon is implemented, and physical constraints are included to realistically restrain the colon deformations. \textit{Unity3D} is adopted for creating high quality and realistic visual rendering including additional visual effects such as reflection on the organ surface or vignetting the
% peripheral darkening of the endoscopy image \cite{incetan2021vr}. 

\textit{Endoscope simulation} - 
We assume a scenario close to active capsule endoscope navigation or robotic endoscope with soft tether with actuation at the tip. Hence, we model the endoscope tip as a rigid capsule with camera, with weight, length and diameter of 20g, 36mm, and  14mm, respectively \cite{wang2021learning}. 

% We assume a scenario close to a magnetically guided FE where external magnets control the motion of the magnetic tip while the tether follows the tip passively \cite{taddese2016nonholonomic}. Hence, in this preliminary simulator version, we neglect the effect of the endoscope tether due to multiple collision points with the colon model that could lead to simulation instability. 
% The endoscope tip is modeled as a rigid capsule with weight, length and diameter of 20g, 36mm, and  14mm, respectively \cite{wang2021learning}. An angular drag of 4 rad/sec$^2$ is added to account for the frictional resistance \cite{wang2021learning}.
% The endoscope tip embeds a camera and has four degrees of freedom for the motion as shown in Fig.~\ref{fig:frame}, i.e., translation (insertion/retraction), roll, and bending in two perpendicular directions (pitch/yaw).


While the assumption of using the region of greatest depth with any given images as the goal for immediate heading adjustment is reasonable \cite{lazo2022autonomous, martin2020enabling, prendergast2018autonomous}, it suffers from a fundamental flaw. The lighting conditions, focal length, and surrounding tissue geometry can greatly affect the actual distance to the maximum depth goal, making it an unreliable target for precise navigation. An algorithm solely based on perfect alignment of the camera towards the deepest point ignores the 3-D structure of the surrounding anatomy will inherently limit the ability of the scope at tight bends (Depicted in Fig.~\ref{fig:image_segmentation}), where a large proportion of images will not be well-centered within the lumen (Depicted in Fig.~ xxx). 
This results in close-up views of the lumen wall that is extremely bright due to reflection. 
Hence, defining safety objectives to avoid the movement of the scope in the orthogonal direction of the colon wall which could potentially lead to perforation, can lead to a safer trajectory.


Therefore, we define two safety metrics:
(1) Soft constraints which provides a guidance for avoiding colon wall collisions based on safety probability analysis and optimization. 
One of the objectives of this study is to incorporate soft constraints during the training of standard DRL methods so that the agent learns to execute action lying in the safe configuration, called constrained RL.
(2) Hard constraints that strictly require the system to not reach certain specified unsafe regions, for instance perforation. We identify that the movement of the scope towards the bright region of the image leads to a trajectory orthogonal to the wall. Hence, we design a set of four hard constraints (called safety properties) that provide a threshold based on the brightness values of different regions of the image. If the values are above the threshold, the robot should restrict its actions in that direction. 

% : which seek to minimise the number of wall collisions. In clinical practise, clinicians tend to use the lumen wall as support to propel the scope tangentially, during difficult manouvers.
% Although this type of behavior is allowed, the purpose of our safe framework is to reduce as much as possible the number of times this condition occurs. One of the objectives of this study is to incorporate the soft constraints during the training of standard DRL methods so that the agent learns to execute action lying in a safe configuration.
% (2) Hard constraints: 

% Therefore, we incorporate two safety metrics: soft and hard constraints. In more detail, the soft constraint seeks to minimize the number of touches the wall in a tangentially fashion. Intuitively this is a soft constraint since, as the endoscopist leans against the walls, even the agent is sometimes allowed to rub against the walls of the colon to make particularly sharp bends. Although this type of behavior is allowed, the purpose of our safe framework is to reduce as much as possible the number of times this condition occurs. Hence, the objective of this study is to incorporate the soft constraints during the training of standard DRL methods so that the agent learns to execute action lying in a safe configuration. However, as mentioned above, the use of constrained DRL methods does not provide any formal guarantee on the behavior of our agent. To this end, we design a set of four additional hard constraints (i.e., safety properties) in order to check and select the model that does not perform orthogonal collisions with the wall. The latter types of collisions are particularly dangerous because they increase the likelihood of perforation of the colon wall and, therefore, should be avoided.


%Safety properties refer to input-output relationship in the domain of interest formalised as follows:

%  \begin{equation} \label{eq:standard_proeprty}
% \Theta:  x_0\in[a_0, b_0] \land ... \land x_n\in[a_n, b_n] \Rightarrow y_j\in[c, d]
% \end{equation}
% \noindent where $x_k \in X$ (i.e., input space), with $k \in [0, n]$, where n denotes the size of input states (i.e. dimension of $X$) and $y_j$ is a generic output of the network. Here, $ a_k, b_k, c, d \in \mathbb{R}$ represents the input and output bounds, respectively.

widely considered the state-of-the-art and one of the most effective algorithms for control problems \cite{schulman2017proximal}. PPO can be implemented following different approaches and optimizations; for our experiments, we rely on an actor/critic architecture, following the guidelines of OpenAI's Spinning Up \cite{achiam2018spinning}.

The observation space consists of a low-dimensional discretization of the endoscopic image into a 4x4 matrix (Shown in Fig.~\ref{fig:observation_space}). The image is discretized by dividing each dimension of the image into four regions such that the each square region is assigned a value which is the average of underlying pixels. The step of discretization is carried out to simplify the definition of safety properties and to preserve the local features in the image. The 2-D down-scaled image is flatted into a list of 16 values.

The action space consists of five discrete actions. Intuitively, each action encodes a movement in the cardinal directions, namely \texttt{forward}, \texttt{left}, \texttt{right}, \texttt{up}, and \texttt{down}. More formally, our agent moves with a constant linear velocity of \SI{3}{\milli\meter/\second}. 
The angular velocity depends on the corresponding action and corresponds to a rotation of a fixed angle (i.e., \SI{0.017}{\radian/\second}) in the two degrees of freedom at the endoscope tip. Considering the input space discussed in the previous section, the neural network controller is shaped with 5 output neurons (i.e., one for each discrete action) and 16 input nodes.

\subsection{Deep Reinforcement Learning (DRL)}
The colon navigation problem is formalized into a Markov Decision Process (MDP) represented by a tuple $(\mathcal{S}, \mathcal{A}, \mathcal{R}, \mathcal{P}, \gamma, T) $, where $\mathcal{S}$ denotes the state space, $\mathcal{A}$ is the action space, $\mathcal{P}$ is the transition probability distribution, $\mathcal{R}$ is the reward space, $\gamma \in [0, 1]$ is the discount factor and $T$ is the time horizon per episode. At each timestep $t$, the environment produces a state observation $s_{t} \in \mathcal{S}$. The agent then generates an action $a_t \in \mathcal{A}$ according to a policy $a_t \sim \pi(s_t)$, and applies it to the environment to receive a reward $r_t \in \mathcal{R}$ \cite{sutton2018reinforcement}. As a consequence, the agent transitions to a new state $s_{t+1}$ sampled from the transition function $p(s_{t+1} | s_{t}, a_{t})$, $p \in \mathcal{P}$ or terminates the episode at state $s_{T}$. The objective of a DRL algorithm is to find a policy that maximizes the expected cumulative reward over a trajectory, more formally:
\begin{equation}
	\label{eq:maximization_drl}
	\max_{\pi_\theta \in \Pi} J_{r}({\pi_\theta}) := \mathbb{E}_{\tau \sim \pi_\theta}[R(\tau)]
\end{equation}

In the previous sections, we introduced the concept of optimal policy for an MDP. However, for safety-critical, an agent is typically required to guarantee additional behaviors that, in some cases, may assume an even greater level of importance than the accomplishment of the task \cite{RaAcAm19}. 
For instance, in colonoscopy, avoiding lumen wall perforation is more critical than reaching the destination, despite the fact that the latter is the primary goal.
% To provide an intuition for an autonomous driving car, avoiding a crash is more important than reaching the destination, despite the fact that the latter is the primary goal.

In literature, this kind of problem is typically modeled through a Constrained Markov Decision Process (CMDP) \cite{Al99}, an extension of a standard MDP which includes an additional signal, the \textit{cost function}, defined as $C: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$, and a threshold $d \in \mathbb{R}$ value which the expected value of the cost must remain below. For simplicity, we assume the case with only one cost function and the corresponding section; however, the framework can be easily extended to handle multiple constraints \cite{RoGiRo21}. More formally, we define the set of feasible policies for a CMDP as follows: 


One possible approach to encode the constraints into an optimization problem is using \textit{Lagrange multipliers}. Specifically, in DRL, a possible approach is to transform the constrained problem into the corresponding dual unconstrained version \cite{LiDiLi20, AcHeTa17}. The objective function for the optimization, which can be maximized with potentially any policy gradient algorithm \cite{StAcAb20}, can be encoded as follows: 


%%%%%%%%%%%%%%%%% Formal verification text %%%%%%%%%%%%%%%%%%%%%

% Although Deep Neural Networks (DNNs) are powerful approximation functions and using Constrained DRL approaches allows the policy to be oriented in safer areas, we still have no formal guarantee that our agent's behavior is completely safe in every situation. 
% In particular, it is known that DNNs are vulnerable to small perturbations of the input space, which could result in incorrect harmful predictions\cite{adversarial}. 
The FV of DNNs \cite{Liu, Reluplex} involves checking whether a particular input-output relationship holds for a given DNN.
Formally, an instance of a DNN-Verification problem consists of a tuple $\mathcal{R}=\langle\mathcal{F}, \mathcal{P}, \mathcal{Q}\rangle$, where $\mathcal{F}$ is a trained DNN, $\mathcal{P}$ is a precondition on the input, and $\mathcal{Q}$ is a postcondition on the output. The predicate $\mathcal{P}$ defines the possible input configurations we are interested in, while $\mathcal{Q}$ represents the output results we aim to guarantee formally for at least one of the inputs that satisfy $\mathcal{P}$. In general, the precondition can be expressed with any geometry, and we use a set of hyper-rectangles (or intervals) to define $\mathcal{P}$.

The verification algorithm then searches and returns $\texttt{SAT}$ if such an $\Vec{x}$ exists in the input space represented by $\mathcal{P}$, and $\texttt{UNSAT}$ otherwise \cite{Verinet1}. Generally, the postcondition encodes the negation of the safety property, representing the action that the agent should avoid. Therefore, if the verifier returns a $\texttt{SAT}$ answer, it indicates that the agent is not safe in the situation encoded in $\mathcal{P}$ since there exists at least one configuration that satisfies $\mathcal{P}$ and for which the agent performs the harmful action.

% Solving the verification problem requires showing that the following assertion holds:
% \begin{equation}
%    \exists\;\Vec{x}\;|\;\mathcal{P}(\Vec{x}) \wedge \mathcal{Q}(\mathcal{F}(\Vec{x}))
% \end{equation}
%  % \[\exists\;x\;|\;\mathcal{P}(\Vec{x}) \wedge \mathcal{Q}(\mathcal{F}(\Vec{x}))\]
% The verification algorithm then searches and returns $\texttt{SAT}$  if exists at least a single concrete input (vector) $\Vec{x}$ that satisfies the given constraint,  $\texttt{UNSAT}$ if no such $\Vec{x}$ exists in the whole input space represented by $\mathcal{P}$. Broadly speaking, the postcondition encodes negation of the safety property, i.e., the action the agent should not perform. Hence, if the verifier returns a $\texttt{SAT}$ answer, this implies that the agent in the situation encoded in the precondition $\mathcal{P}$ is not safe since it exists at least one configuration that satisfies $\mathcal{P}$ and for which the agent performs the harmful action.

% Using the input values for $\mathcal{F}$ (depicted in Fig.~\ref{fig:observation_space}b) as an indicative metric, and $y_0,...,y_4$ five possible actions that the agent can choose, we define a set of four safety properties, namely $\Theta_{\downarrow}, \Theta_{\uparrow}, \Theta_{\rightarrow}, \Theta_{\leftarrow}$. The formulation and description of these properties are elaborated in Tab.~\ref{tab:safety_props}, where $x_0,...,x_{15} \in \Vec{x}$ are a set of possible values in the intervals which represent the precondition $\mathcal{P}$ with $x_0$ that represents the value of the upper left and $x_{15}$ the bottom right square respectively. 
% The interval $[0, 0.6]$ encodes a safe situation in that the image area is dark and therefore free of possible obstacles, while the interval $[0.8, 1]$ encodes the opposite situation, a clear image area, i.e., the agent is near the colon wall.
% We express the postcondition $\mathcal{Q}$ such that the agent should choose any action different from $y_2$, which encodes the unsafe action corresponding to the movement of the scope in the direction of illumination. The properties defined are symmetric in nature.
% To verify the properties, a formal verification tool searches for a single input configuration $\Vec{x}$ that satisfies $\mathcal{P}$ and the negation of the postcondition, i.e., $\bigwedge_{i=0,1,3,4} y_i \leq y_2$, i.e., a situation for which the agent selects the unsafe action $y_2$. If no such configuration is found, the original property holds.
% These properties, if formally satisfied, will ensure that the agent will not perform actions that lead to colon wall perforation.

An important thing to note is that the safety properties specify the unsafe action not to take, but do not specify which other action to take. This is because our purpose is to formally verify that in an unsafe situation, the most harmful action should never be taken. 

% For the postcondition $\mathcal{Q}$, we express the condition in which the agent should choose any action different with respect to $y_2$ that encodes the unsafe action corresponding to a downward movement. Hence, to verify this property, a formal verification tool searches for a single input configuration $\Vec{x}$ that satisfies $\mathcal{P}$ and the negation of the postcondition, i.e., $\bigwedge_{i=0,1,3,4} y_i \leq y_2$, i.e., a situation for which the agent selects the unsafe action $y_2$. If no such configuration is found, the original property holds.
% These properties, if formally satisfied, will ensure that the agent will not perform actions that lead to colon wall perforation.


% As an example of how a safety property can be expressed in this context, let us consider the situation depicted in Fig. \ref{fig:observation_space}a. We note that the agent is located very close to the lower part of the colon; in fact, the portion of the colon is strongly illuminated by the capsule as the lower part of the image is completely white. In this situation, we want to formally verify that our agent never selects the action corresponding to a downward movement, which would correspond to an orthogonal collision with the colon. 
% Using the input values for $\mathcal{F}$ (depicted in Fig.~\ref{fig:observation_space}b) as an indicative metric, and $y_0,...,y_4$ five possible actions that the agent can choose, we can define the following property:
% As an example of how a safety property can be expressed in this context, considering the possible input values for $\mathcal{F}$ shown in Figure~\ref{fig:observation_space}b, and considering the five potential actions $y_0,...,y_4$ that the agent can take, we can design the following property:
% % \begin{equation}
% \begin{align*}
% x_0,...,x_{11} \in [0, 0.6]\;\wedge \;
% & x_{12},...,x_{15} \in [0.8, 1.0] \notag \\
% &\Downarrow\\
% \bigvee_{i=0,1,3,4} &y_i \geq y_2
% \end{align*}
% % \end{equation}

% where $x_0,...,x_{15} \in \Vec{x}$ are a set of possible values in the intervals which represent the precondition $\mathcal{P}$ with $x_0$ that represents the value of the left upper and $x_{15}$ the right bottom square respectively. For the postcondition $\mathcal{Q}$, we express the condition in which the agent should choose any action different with respect to $y_2$ that encodes the unsafe action corresponding to a downward movement. Hence, to verify this property, a formal verification tool searches for a single input configuration $\Vec{x}$ that satisfies $\mathcal{P}$ and the negation of the postcondition, i.e., $\bigwedge_{i=0,1,3,4} y_i \leq y_2$, i.e., a situation for which the agent selects the unsafe action $y_2$. If no such configuration is found, the original property holds.

% \begin{align*}
%         \Theta_{\downarrow}: x_0,...,x_{11} \in [0, 0.6]\;&\wedge x_{12},...,x_{15} \in [0.8, 1.0]\rightarrow y \neq y_{\downarrow}
% \end{align*}

% where the interval $[0, 0.6]$ encodes a safe situation in that the image area is dark and therefore free of possible obstacles, while the interval $[0.8, 1]$ encodes the opposite situation, a clear image area, i.e., the agent is near the colon wall. With this encoding, it is possible to express four symmetric properties, i.e., whether the agent is near the upper or lower wall, left or right side of the colon, it does not have to perform an action orthogonal to the direction of the wall. The important thing to note is that the safety properties specify the most dangerous action not to take, but do not specify what other action to take. This is because our purpose is to formally verify that in an unsafe situation, the most harmful action should never be taken. Hence, another action that could lead to touch with the surface of the colon could be accepted in order to take a safer trajectory.

% Here, $\Vec{x} = {x_0,...,x_{15}}$ is a set of intervals that represents the precondition $\mathcal{P}$, with $x_0$ and $x_{15}$ respectively denoting the value of the left upper and right bottom square. The postcondition $\mathcal{Q}$ specifies that the agent should not choose the unsafe action corresponding to a downward movement, which is represented by $y_2$. To verify this property, a formal verification tool searches for an input configuration $\Vec{x}$ that satisfies $\mathcal{P}$ and for which the agent selects the unsafe action $y_2$. If no such configuration is found, the negation of the postcondition, i.e., $\bigwedge_{i=0,1,3,4} y_i \leq y_2$, is deemed satisfied.


%%%%%%%%%%%% Experimental Validation%%%%%%%%%%%%%
In the next sections, we show the empirical evaluation of our framework. In particular, our experiments aim to answer the following questions: (Q1) \textit{what impact does a constrained approach have on agent training and its performance in the autonomous colon navigation task?} 
% (Q2) \textit{what is the difference between our novel encoding of the input space and the classical use of lumen distance?} 
(Q2) \textit{can lowering the violation of soft constraints directly 
% imply lowering or completely zeroing 
eliminating the violation of hard constraints? } 

% In particular, both implementations used the same architecture consisting of two hidden layers with 64 units each and activated with ReLU to model actors and critic networks, respectively. Moreover, the same reward function introduced in Sec. \ref{eq:methods:reward_function} is used.

% In order to analyze the statistical significance of the data \cite{colas2019hitchhikers}, we trained 300 models for each methodology using one of the colon models $C_1$ for training and the other three for the evaluation phase. Data are collected on a RTX 2070, and an i7-9700k, reporting the mean and standard deviation gathered from ten independent runs.

% In order to answer the last question, we perform the formal verification on the 300 models trained for each methodology. In particular, we have designed a set of four safety properties that aim to control that the agent does not perform actions that lead to a colon wall perforation situation. In more detail, the properties are of the following form:

% To answer Q2, FV of the 300 models trained for each methodology is performed. 
% We design a set of four safety properties, namely $\Theta_{\downarrow}, \Theta_{\uparrow}, \Theta_{\rightarrow}, \Theta_{\leftarrow}$ which if formally satisfied, the agent will not perform actions that lead to colon wall perforation.

% \begin{align*}
%         \Theta_{\downarrow}: x_0,...,x_{11} \in [0, 0.6]\;&\wedge x_{12},...,x_{15} \in [0.8, 1.0]\rightarrow y \neq y_{\downarrow}
% \end{align*}

% where the interval $[0, 0.6]$ encodes a safe situation in that the image area is dark and therefore free of possible obstacles, while the interval $[0.8, 1]$ encodes the opposite situation, a clear image area, i.e., the agent is near the colon wall. With this encoding, it is possible to express four symmetric properties, i.e., whether the agent is near the upper or lower wall, left or right side of the colon, it does not have to perform an action orthogonal to the direction of the wall. The important thing to note is that the safety properties specify the most dangerous action not to take, but do not specify what other action to take. This is because our purpose is to formally verify that in an unsafe situation, the most harmful action should never be taken. Hence, another action that could lead to touch with the surface of the colon could be accepted in order to take a safer trajectory.


To demonstrate the effectiveness of the proposed framework, we consider four patient-specific colon models with equivalent complexity. The model complexity is characterized by the centerline from the rectum to the colon end, and the number of acute bending, i.e., >90 degrees, estimated through visual inspection. Our first experimental goal is to check the training differences between PPO and L-PPO. Hence, 300 policies for each methodology was trained on one of the colon model to provide statistical significant data.
The other three models were used for evaluation phase. Data are collected on a RTX 2070, and an i7-9700k, reporting the mean and standard deviation gathered from ten independent
runs.


Learning curves of PPO and L-PPO are compiled in Fig.~\ref{fig:training_results}a. We note an equivalent performance in the learning curves of the two algorithms, which reach higher reward values at ~400 episodes.

We find that L-PPO is successful at enforcing constraints as it tracks the constraint cost below the limit value at 300 episodes while PPO constraint cost stays above the limit. This suggests that L-PPO can find a policy which on average satisfies approimate constraints better than PPO.

We observe that both PPO and L-PPO reach 100\%  success in navigating all the colon models i.e. both the algorithms can reach the end of the colon. We present the average distance travelled by the scope for each patient colon in Table.~\ref{tab:centerline_results}, where comparison between L-PPO, PPO and PPO$_{lum}$ is carried out. PPO$_{lum}$ represents PPO trained using the lumen centralisation reward function proposed in previous work by \cite{pore2022colonoscopy}. Average distance travelled is crucial in evaluating the trajectories since multiple backward motions or reversing the direction of motion can lead to suboptimal trajectories.
The distance travelled is measured using the position values of the endoscope tip normalised by the centerline distance of the colon model.
We note an equivalent performance for all the three algorithms, indicating that DRL can be trained without lumen centralisation reward over a global objective of reaching the colon end. The values indicate that a shorter path than the centerline is followed.


To answer Q2, FV of the 300 models trained for each methodology is performed. 
Table \ref{tab:formal_verification} shows the violations for PPO and L-PPO, for all four safety properties respectively. Specifically, two columns $\texttt{SAT}$ and $\texttt{UNSAT}$ are reported for each property, representing the number of models that violate or do not violate that particular safety property. In particular, we can see that for the first property $\Theta_\uparrow$, which encodes the situation where if the upper part of the image is very bright the agent does not have to take an upward action, all 300 PPO models violate the property. We can motivate this behavior since in all 4 colon models used, the tight bends are not only to the left or right but also upward and downward, and thus an approach that does not incorporate soft constraints into the training is unlikely to learn to avoid these risky situations.

The table shows that L-PPO generally exhibits fewer violations than PPO, indicating that the inclusion of soft constraints in training leads to a decrease in violations of hard constraints.

%%%%%%%% COnclusion %%%%%%%%%

% In this work, we address the safety challenges of deploying DRL for navigating the colonic tract in a virtual simulation.
% DRL methods can successfully navigate patient-specific colon model with performance comparable to expert clinicians \cite{pore2022colonoscopy}. However, these methods are vulnerable to adversarial attacks which could lead to safety violations. Even if such violations are rare, they can have fatal consequences. 
% Hence, we exploit a constrained-RL methodology, that encodes soft safety constraints through a cost function of safety violations. Our results indicate that constrained-RL reduces the policy search space to where the expectation of cumulative discounted cost is less than a threshold. 
% However, it is challenging to enforce hard constraints using the constrained RL methodology. Therefore, we develop a model selection strategy, where a vast repertoire of policies are trained using constrained-RL, and their safety is evaluated by leveraging FV.
% The formal verification is a modular framework that can verify the violation against any given set of safety properties and provide guarantees of a safe behaviour, prior to deployment.
% Out of the 300 policies trained using constrained RL, we found 3 policies that follows all the safety constrained being completely safe as opposed to 0 policies being completely safe for standard DRL

==> table.tex <==
% \begin{table*}
% \centering
% \vspace{15pt}
% \caption{Comparison between $DVC_{C_0}$ and $DVC_{C_{0} + C_{1}}$}
% \label{Tab:abb}
% \begin{tabular}{ c c c c c c c c c c c c }
% \hline\noalign{\smallskip}
%       & \multicolumn{4}{c}{$DVC_{C_0}$} && \multicolumn{4}{c}{$DVC_{C_{0}+C_{1}}$} \\
% \noalign{\smallskip }\cline{2-5} \cline{7-10} \noalign{\smallskip} 
%       & \makecell{Average\\LD} & CWC & TOI & \makecell{Normalised \\ distance} && \makecell{Average\\LD} & CWC & TOI & \makecell{Normalised \\ distance} \\
% \noalign{\smallskip}\hline\noalign{\smallskip}
% $C_0$ & 0.27$\pm$0.01 & 0.5$\pm$0.25 & 1.37$\pm$0.05 & 0.84$\pm$0.02 && 0.24$\pm$0.02 & 1$\pm$1 & 1.32$\pm$0.03 & 0.84$\pm$0.02 \\
% $C_1$ & 0.30$\pm$0.01 & 3.3$\pm1.5$ & 1.74$\pm$0.04 & 0.88$\pm$0.08 && 0.25$\pm$0.01 &  3.3$\pm$0.5 & 1.70$\pm$0.07 & 0.82$\pm$0.03  \\
% $C_2$ & 0.36$\pm$0.03 & 5$\pm$1 & 2.22$\pm$0.2 & 0.97$\pm$0.03 && 0.28$\pm$0.01 & 4.6$\pm$0.5 & 1.89$\pm$0.03 & 0.85$\pm$0.01 \\
% $C_3$ & 0.35$\pm$0.02 & 4.6$\pm$0.5 & 2.15$\pm$0.23 & 0.92$\pm$0.08 && 0.29$\pm$0.03 & 3$\pm$1 & 1.78$\pm$0.05 & 0.89$\pm$0.09  \\
% % C4 & 0.29$\pm$0.02 & 6$\pm$0.8 & 1.95$\pm$0.15 & 0.90$\pm$0.02 && 0.21$\pm$0.03 & 6.3$\pm$0.5 & 1.85$\pm$0.01 & 0.88$\pm$0.02 \\
% % C5 & 0.33$\pm$0.01 & 7.3$\pm$0.6 & 3.8$\pm$0.35 & 0.95$\pm$0.02 && 0.27$\pm$0.01 & 6.3$\pm$0.66 & 3.3$\pm$0.2 & 0.97$\pm$0.03 &  \\
% % C6 & 0.21$\pm$0.01 & 4.3$\pm$0.5 & 1.55$\pm$0.05 & 0.89$\pm$0.02 && 0.15$\pm$0.02 & 3.3$\pm$0.5 & 1.46$\pm$0.04 & 0.85$\pm$0.02 \\
% % C7 & 0.33$\pm$0.04 & 5.6$\pm$0.5 & 2.72$\pm$0.16 & 0.86$\pm$0.02 && 0.22$\pm$0.02 & 4.3$\pm$0.5 & 2.26$\pm$0.15 & 0.84$\pm$0.01 \\
% % C8 & 0.33$\pm$0.03 & 4.6$\pm$0.3 & 1.50$\pm$0.05 & 0.86$\pm$0.01 && 0.21$\pm$0.03 &  4$\pm$0 & 1.51$\pm$0.03 & 0.85$\pm$0.02 \\
% \hline
% Mean & 0.31$\pm$0.04 & 5.0$\pm$1.2 & 2.20$\pm$0.75 & 0.90$\pm$0.04 && \textbf{0.23$\pm$0.04} & \textbf{4.3$\pm$1.2} & \textbf{1.96$\pm$0.59} & \textbf{0.86$\pm$0.04} \\
% \noalign{\smallskip}\hline
% \end{tabular}
% % \vspace{-15pt}
% \end{table*}



==> table2.tex <==
% \begin{table}
% \centering
% \caption{NASA Task Load Index for novice users.}
% \label{Tab:task}
% \begin{tabular}{ c c c c }
% \noalign{\smallskip }\hline\noalign{\smallskip}
% % \cline{2-5} \cline{7-10} \noalign{\smallskip} 
%  & \makecell{Manual\\control} & \makecell{Rule-based\\control} & DVC \\
% \noalign{\smallskip}\hline\noalign{\smallskip}
% Mental demand & 63 & 33 & \textbf{18}\\
% Physical demand & 65 & 38 & \textbf{9} \\
% Temporal demand & 30 & 47 & \textbf{17} \\
% Performance & 25 & 34 & \textbf{12}  \\
% Effort & 57 & 38 & \textbf{10}  \\
% Frustration & 42 & 41 & \textbf{12} \\
% Mean workload & 47 & 38 & \textbf{13} \\
% \noalign{\smallskip}\hline
% \end{tabular}
% % \vspace{-15pt}
% \end{table}

==> table3.tex <==
% \begin{footnotesize}
% % \begin{small}
% \begin{table*}
% \centering
% \vspace{15pt}
% \caption{Navigation parameters used for validation with their description} \label{tab:autonomy_table} 
% % \begin{tabular}{ c c c }
% \begin{tabular}{p{0.3cm}p{2cm}p{13.8cm}}
% % \hhline{|=|=|=|=|=|}
% \noalign{\smallskip }\hline\noalign{\smallskip}
%  & \makecell{Navigation\\metrics} & Description \\
% \toprule
% 1 & Time of insertion (TOI) & TOI is measured from the time point where the initial movement of the endoscope is detected to the time point when the caecum is reached. \\
% \midrule
% 2 & Colon Wall Collision (CWC) & CWC refers to the scenario when the endoscope tip touches the colon wall. The average diameter of the colon models used is 5cm, hence a threshold of $\delta d = 1cm$ is decided to classify the deformation as CWC.\\
% \midrule
% 3 & Normalised distance & Distance travelled is crucial as multiple backward motions, reversing the direction, can lead to suboptimal trajectories.
% The distance travelled is measured using the position values of the endoscope tip. This distance is normalised by the centerline distance of the colon model in order to compare among different colon models. Normalised distance above 1 indicates a path distance longer than the centerline path, while a normalised distance below 1 indicates a shorter path than the centerline was followed. \\
% \midrule
% 4 & Average Lumen Distance (LD) & Lumen centralisation is believed to create smooth insertion trajectories hence the lumen distance in the image plane is recorded at each timepoint. This distance is normalised by the size of the image to get a value in [0,1]. Lumen distance value 0 denotes image centre ($P_c$) coincides with the detected lumen ($P_L$), and value 1 denotes that the detected lumen is at the farthest point. \\
% \midrule
% % \hhline{|=|=|=|=|=|}

% \end{tabular}
% % \vspace{-15pt}
% \end{table*}
% % \end{small}
% \end{footnotesize}
